SMS Goes Nuclear: Fortifying SMS-Based MFA in Online Account Ecosystem

With the rapid growth of online services, the number of online accounts proliferates. The security of a single user account no longer depends merely on its own service provider but also the accounts on other service platforms(We refer to this online account environment as Online Account Ecosystem). In this paper, we first uncover the vulnerability of Online Account Ecosystem, which stems from the defective multi-factor authentication (MFA), specifically the ones with SMS-based verification, and dependencies among accounts on different platforms. We propose Chain Reaction Attack that exploits the weakest point in Online Account Ecosystem and can ultimately compromise the most secure platform. Furthermore, we design and implement ActFort, a systematic approach to detect the vulnerability of Online Account Ecosystem by analyzing the authentication credential factors and sensitive personal information as well as evaluating the dependency relationships among online accounts. We evaluate our system on hundreds of representative online services listed in Alexa in diversified fields. Based on the analysis from ActFort, we provide several pragmatic insights into the current Online Account Ecosystem and propose several feasible countermeasures including the online account exposed information protection mechanism and the built-in authentication to fortify the security of Online Account Ecosystem.

==> Background.tex <==
% !TEX root = main.tex
%1page
\section{Background}
\label{sec:motivation}

%{\bfseries{Online Account Service.}}
%An online account allows a user to authenticate to an online service and potentially to receive authorization to access resources provided by or connected to that online service. To log into an online account, a user is typically required to authenticate oneself with a password or other credentials for the purposes of accounting, security, logging, and resource management.
\squishlist
\item{\bf{SMS-based Account Authentication.}}
SMS-based account authentication has been widely accepted in recent years~\cite{PhoneFactor,SMS,Google}. To ensure the security of login process, most of the online service provides users with SMS Code through telecom operator channels. 
The process of SMS-based account authentication mainly consists of five steps. Firstly, the user sends SMS verification request on the webpage to the server of the Internet service provider. Secondly, the server generates a series of random numeric string and sends it to the SMS platform. Then, the SMS platform sends the numeric string to the user's cellphone through the telecom operator channel. After the user receives the SMS, he/she submits the numeric string to the server. Finally, the server matches the consistency of the numbers (shown in Fig.~\ref{Fig:smsauth}).

%The SMS-based authentication spreads rapidly due to the tremendous development of mobile Internet service. The cellphone users naturally own the phone numbers with only a limited amount. In some countries, e.g. China, real-name registration has been legitimated to map the mobile number to the specific person. Thus, the Internet service provider can ensure the uniqueness of the account owners. Besides, SMS-based authentication has the advantages of easy deployment, low cost, and no additional equipment, which makes it as the preferred choice of major Internet service providers.    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.35\textwidth]{smsauth0615}
%	\vspace{-0.06in}
    \setlength{\abovecaptionskip}{-1pt}
	\caption{Diagram of SMS-based Authentication.} 
	\vspace{-0.5cm}
	\label{Fig:smsauth}	
\end{figure}       
%at the very beginning, some use password+username, password+ username & SMS code, password + username + E-key, phone number + SMS Code


\item{\bf{Online Account Personal Information.}}
When users enjoy the convenience of online services, e.g., online shopping, the Internet service providers always try to collect as much information from their users as they can and store the personal information in their servers. For example, E-commerce platform stores the usernames, cellphone numbers, e-mail addresses, delivery addresses, order records, wish lists and payment information on the "Your Account" page. The exposed personal information can be divided into 4 categories, i.e., individual basic information (e.g. real name, cell phone number, e-mail address, ID number or social security number, driving license, and address), account information (e.g. username, user ID, bonded account, bonded bankcard number, and bonded cellphone number), privacy records (e.g. contact list, chat list, text files, media, orders and wish list), and social relationship information (e.g. friend list, parents, and workplace).


% This can improve the user online shopping experience and help the platform provide customized service. However, the personal information is exposed without any masking here and anyone who successfully logs into the account can retrieve it easily.



\squishend
%{\bfseries{OsmocomBB-based SMS sniffing.}}





%\xxx realizes the goals of high-speed and inaudibility by utilizing the nonlinearity effect of microphones. In this section, we first describe the microphone system in mobile devices, and then elaborate the nonlinearity effect.

% \subsection{Acoustic Communications}
% Without requiring specific hardwares like RF, bluetooth or NFC chips, the acoustic communication provides a lightweight method for data transmission with speakers and microphones. One of the main advantages of the acoustic communication is that this technique does not need devices paring or human intervention in advance, and an increasing number of applications utilize this communication method for the small file exchanging or handshaking. For example, AliPay allows ``acoustic pay'' for easy checking out nowadays. In the acoustic communication, binary files are first modulated into acoustic waves with various frequencies, e.g., utilizing $ 900Hz $ and $ 1.5kHz $ acoustic waves to represent ``1'' and ``0'' separately. The modulated acoustic waves are transmitted through a speaker and received by a targeted device with a microphone. This process usually lasts for several seconds depending on the length of the file. With the received acoustic waves, the file will be demodulated according to a predefined modulation rule. %By checking the CRC bit or utilizing other data verifying methods, one acoustic communication is finished. 
% Even though acoustic communication are used in many applications, there are still several limitations exist. For example, the acoustic wave is audible to humans, and higher frequency of acoustic waves bring unpleasant user experiences. Basing on this, proposing an efficient and inaudible acoustic communication is crucial.
%On the other hand, to enhance the accuracy of data transmission, the transmission power is also set at an annoying level, which also suppress the enthusiasm of users. Basing on this, an efficient and inaudible acoustic communication may solve the problems above. 


%\subsection{Microphone System}
%A microphone system converts acoustic waves into electrical signals. Microphones on mobile devices can be either Electret Condenser Microphone (ECM) or Micro Electrical Mechanical System (MEMS). Nowadays, MEMS microphones dominate the market of mobile devices such as smartphones, Pads and wearable devices like smart watch due to the miniature package sizes and low power consumption. Thus, we focus mainly on MEMS microphones in this paper yet the analysis suits for both MEMS and ECM microphones. 
% The most common types of microphones are the Electret Condenser Microphone (ECM), which utilizes a capacitor plate to sense the vibration, and the piezoelectric microphone with a crystal piezoelectric material to produce voltage when subjected to pressure. However, due to the requirements of packaging and power consumption in mobile devices, the 
% Thus, we propose an inaudible channel communication method which mainly focuses on MEMS microphones.
%\subsubsection{Throughput}
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.4\textwidth]{structureMEMS}
%	\caption{Struture of MEMS microphone.} 
%	\label{Fig:MEMS}	
%\end{figure}
%As shown in Fig.~\ref{Fig:MEMS}, the MEMS microphone contains a membrane and a fixed back plate electrode. When a sound wave comes, it passes through the air gap between the back plate electrode and reaches the membrane. The membrane bends With the changed air pressure caused by the sound wave, and the electric capacity between the membrane and the fixed back plate electrode is also changed and captured by the ASIC unite (Application Specific Integrated Circuit). In this way, MEMS microphone covert the sound wave into the electrical signal.

%In order to capture audible sounds, microphones, low-pass filters (LPFs), and analog-to-digital converter (ADC) in the microphone system are used to suppress signals out of the frequency range of audible sounds (i.e., 20 Hz to 20 kHz). The typical structure of microphone is shown in Fig.~\ref{Fig:nonlinearity_model}.
%Most sound communication systems are constrained by the belief that sound communication can only be in audible frequency band due to suppression of signals above 20 kHz. 
% The nature uses of the microphone is recording the audible sound with the frequency from $20Hz$ to $20kHz$ and signals at high frequencies shall be filtered by a LPF (low-path filter). 
% After passing through the LPF, an ADC is added to covert digital signals to analog signals for further analysis. 
% The typical sampling rate of the ADC is $44.1kHz$, and according to the Shannon sampling theorem, the frequency of the digital signal is limited below $22kHz$.

%\subsection{Nonlinearity Effect Modeling}
%% \com{This is not the model for AM.}
%Nonlinearity is a phenomenon that demodulated signals can be produced in low-frequency range. It is reported to appear in many electric components, such as operational amplifiers~\cite{fiori2002nonlinear,chen1980macromodel,kune2013ghost,graffi1991new,fiori2002new}.
%For a microphone, nonlinearity means when a modulated high-frequency signal (e.g. $>$ 20 kHz) passes through the microphone, low-frequency signal (e.g. $<$ 20 kHz) can be generated and received by the microphone. 
%
%Nonlinearity effect has been regarded as distortions of devices and avoided~\cite{wambacq2013distortion}. In \xxx, however, we attempt to exploit the nonlinearity effect to transmit modulated data on frequency above 20 kHz and recover it in the audible frequency band.
%
%
%\begin{figure}[tp]
%	\centering
%	\includegraphics[width=0.48\textwidth]{nonlinearity2}
%	\vspace{-0.06in}
%	\caption{A modulated signal on high frequency carrier ($>$ 20 kHz) is input to the microphone (1) and a new low-frequency ($<$ 20 kHz) signal is generated (2). The new signal as well as other high-frequency are amplified (3) while the high-frequency signals are finally filtered by the LPF (4).} 
%	\vspace{-0.12in}
%	\label{Fig:nonlinearity_model}	
%\end{figure}
%
%
%Without loss of generality, let $S$ be a single frequency signal with a frequency of $f_{S}$. Theoretically, the output signal under nonlinearity effect can be modeled as:
%\begin{equation}
%\label{nonlinearity}
%S_{out} = \left\{
%\begin{array}{ll} \vspace{0.1in}
%a_{0}S&,f_S\le f_{rcv}\\ 
%\sum\limits_{i=1}^{\infty} a_{i}S^{i}&,f_S> f_{rcv}\\
%\end{array} \right.
%\end{equation}
%where %$S$ is a single frequency signal, $f_{S}$ represents the frequency of signal $S$ and 
%$a_{0}$ is the gain coefficient for signals of a frequency less than $f_{rcv}$ and $f_{rcv}$ is the maximum receiving 
%frequency of the receiver. %microphones~\footnote{The value is 22.05 kHz for most smartphones as the sampling frequency is 44.1 kHz.}
%In Eq.~(\ref{nonlinearity}), when $f_{S}>f_{rcv}$, $S_{out} = a_1S+a_2S^2+\dots+a_nS^n$. Typically, the values of $a_{i}, (i \geq 1)$ are related to $f_{S}$, and $a_{i}$ decreases with the increase of $i$. According to the basic trigonometric theory, the frequency of $S^{i}$ is higher than $f_{rcv}$ when $i\ge1$. As a result, the nonlinearity response, i.e., $a_1S^{1}$, $a_2S^{2}$, $a_3S^{3}$, ..., can be eliminated by the LPF in the microphone system. What is more, $a_i$ becomes small when $i\ge3$, thus we often consider the nonlinearity response as $S_{out}=a_1S+a_2S^2$ when $f_{S}>f_{rcv}$.
%
%\textbf{Nonlinearity response for microphone system.} For a microphone system, the nonlinearity effect can be utilized for inaudible communications.
%% with the frequency beyond human capability ($20kHz$). 
%Define an input signal to microphone as $S_{in} = S_{1}(1+S_{2})$ where $S_1=sin\omega_1t$ is the carrier signal with frequency $f_{S_{1}}>f_{rcv}$ and $S_2=sin\omega_2t$ is the baseband signal with frequency $f_{S_{2}}<f_{rcv}$.
%% = sin\omega_1t+sin\omega_2t$ with $f_{s_1}>f_{s_2}>22.05kHz$~\footnote{The value is 22.05 kHz for most smartphones as the sampling frequency is 44.1 kHz.}, 
%According to Eq.~(\ref{nonlinearity}), the nonlinearity response through a microphone $S_{out}$ should be:% (neglect higher-order harmonics):
%\begin{equation}
%\small
%\label{equ:sout}
%S_{out}  = \sum\limits_{i=1}^{\infty} a_{i}(S_1+S_1*S_2)^i
%\end{equation}
%After neglecting the high-order harmonics ($i\ge 3$), $S_{out}$ can be represented as:
%%\begin{equation}
%%\label{equ:nle}
%%\begin{split}
%%S_{out}   &= a_{1}(sin\omega_1t+sin\omega_1t*sin\omega_2t)+\\&  a_{2}(sin\omega_1t+ sin\omega_1t*sin\omega_2t)^2\\
%%&= a_{1}(sin\omega_1t+sin\omega_2t) + a_{2}(1-\frac{1}{2}cos(2\omega_{1}t)-\\
%% &  \frac{1}{2}cos(2\omega_{2}t)+cos((\omega_{1}-\omega_{2})t)-cos((\omega_{1}+\omega_{2})t))\\ 
%%\end{split}
%%\end{equation}
%\begin{equation}
%\label{equ:nle}
%\begin{split}
%S_{out}   &= a_{1}(sin\omega_1t+sin\omega_1t*sin\omega_2t)+\\&  a_{2}(sin\omega_1t+ sin\omega_1t*sin\omega_2t)^2\\
%\end{split}
%\end{equation}
%We then expand Eq.~(\ref{equ:nle}), and the output of the signal contains the baseband signal frequency $f_{S_2}$, the carrier signal frequency $f_{S_1}$, and other harmonics such as $(f_{S_1}-f_{S_2}),~(f_{S_1}+f_{S_2}$) and other cross frequencies (i.e., $2f_{S_1}, 2f_{S_2}, 2(f_{S_1}+f_{S_2}), 2f_{S_1}+f_{S_2}, 2f_{S_1}-f_{S_2}$).
%\begin{figure}[tp]
%	\centering
%	\includegraphics[width=0.42\textwidth]{nonlinearity}
%	\vspace{-0.06in}
%	\caption{Verification of nonlinearity effect. The time and frequency domain response are demonstrated respectively for the original signal, the output signal after a MEMS microphone.} 
%	\vspace{-0.15in}
%	\label{Fig:nonlinearity}	
%\end{figure}
%As mentioned above, the resulting signals from nonlinearity effect with frequency lower than the cut-off frequency of LPF ($f_{LPF}$, which is often set to 25 kHz) will remain while others are filtered. 
%That is to say, the signal $S_2$ ($f_{S_{2}}<f_{rcv}$) modulated on $S_1$ will be reproduced and output from the microphone.
%%That is to say, if $f_{S_1}-f_{S_2}<f_{LPF}$, the signal with frequency of $f_{S_1}-f_{S_2}$ will be produced and output from the microphone. 
%Fig.~\ref{Fig:nonlinearity_model} illustrates the whole process where a signal from nonlinearity effect is generated. 
%
%\subsection{Nonlinearity Effect Validation}
%We conduct an experiment to verify the nonlinearity effect in a microphone. An iPhone SE smartphone is sued to generate a 2 kHz baseband signal. The baseband signal is then inputted to a vector signal generator, which modulates the baseband signal onto a 20 kHz carrier.
%In Fig.~\ref{Fig:nonlinearity}, the top two figures show the original signal from the smartphone, in both time domain and frequency domain, whereby the carrier frequency (20 kHz) and an upper side band as well as a lower sideband ($20 \pm 2$ kHz) can be seen. 
%The bottom two figures show the output from the microphone with. We can clear observe the baseband signal (2 kHz) in the frequency domain. This proves the existence of nonlinearity effect on microphones and the feasibility of transmission by modulating low-frequency signals onto a high-frequency carrier.

% Fig.~\ref{Fig:nonlinearity} is an illustration of the nonlinearity, the lower side represents the process of the signal processing, and the upper side is the FFT of the signals after each procedure. We send signals at different high frequencies which are inaudible to humans. When the signals are received by the microphone, a low frequency is generated due to the nonlinearity as shown in (2). After passing through the amplifier and the LPF ((3) and (4) in Fig.~\ref{Fig:nonlinearity}), the high frequency signals are filtered and the amplified low frequency signal is passed to the AD converter and then decoded by the device. 


%As shown in Fig.~\ref{Fig:nonlinearity}, if we send signals at different frequencies, which are inaudible to humans, a signal with low frequency can pass the LPF and received by the microphone according to the nonlinearity characteristic. The detail of the utilization of the nonlinearity characteristic will be discussed in Sec.~\ref{sec:protocol}.





==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		
